A Comparative Analysis of Ookla Speedtest and Measurement Labs Network Diagnostic Test (NDT7)

Consumers, regulators, and ISPs all use client-based "speed tests" to measure network performance, both in single-user settings and in aggregate. Two prevalent speed tests, Ookla's Speedtest and Measurement Lab's Network Diagnostic Test (NDT), are often used for similar purposes, despite having significant differences in both the test design and implementation, and in the infrastructure used to perform measurements. In this paper, we present the first-ever comparative evaluation of Ookla and NDT7 (the latest version of NDT), both in controlled and wide-area settings. Our goal is to characterize when and to what extent these two speed tests yield different results, as well as the factors that contribute to the differences. To study the effects of the test design, we conduct a series of controlled, in-lab experiments under a comprehensive set of network conditions and usage modes (e.g., TCP congestion control, native vs. browser client). Our results show that Ookla and NDT7 report similar speeds under most in-lab conditions, with the exception of networks that experience high latency, where Ookla consistently reports higher throughput. To characterize the behavior of these tools in wide-area deployment, we collect more than 80,000 pairs of Ookla and NDT7 measurements across nine months and 126 households, with a range of ISPs and speed tiers. This first-of-its-kind paired-test analysis reveals many previously unknown systemic issues, including high variability in NDT7 test results and systematically under-performing servers in the Ookla network.

==> conclusion.tex <==
\section{Conclusion}\label{sec:conclusion}




==> deployment_data.tex <==
\section{Netrics Results}
\label{sec:netrics}
We would already have explained the protocol differences among the speed tests and its impact on the throughput.  Ideally,  this section should focus on the effect of server infrastructure on the results accuracy (and consistency). 

We answer the following questions. 
\begin{itemize}
\item How consistent is a test with itself over time?
\item How consistent are tests with each other?
\item Why do (wired) tests show variability? Understanding the effect of time of the day,  changes in the server,  service upgrade,  speed tiers?
\end{itemize}


\subsection{Consistency over time}
\label{ssec:infra}

I would define this as the fraction of the time that each test achieves is long-term max.
Any single non-maximal result is not necessarily the ``fault'' of the infrastructure, 
  but since the tests run at random times tests that have a markedly reduced probability
  of achieving within 5-10\% of nominal/maximal signal infrastructure rather than user issues.

To do this, we need a baseline maximum across TCP-based tests.
The simple version of this would simply be the max over the study period.
But contracts change over time, so perhaps we have to do the maximum over a day or a week, 
  and reject periods where that rolling maximum is not stable.

This could then put ``nominal speed'' on the $x$-axis and $P(s > 0.9 \times s_\textrm{max})$ on the $y$-axis?

\begin{itemize}
\item can also test high-throughput uplinks from the university or AWS.
\end{itemize}


\subsection{Consistency with other tests}
We show how a test performs with respect to others.  We define consistency relative to the MLab NDT7 test.  More specifically,
\begin{equation}
CT_{test} = Perc_{90} (test) / Perc_{90} (NDT7)  
\end{equation}

Clearly, $CT_{NDT7}$ = 1. A value higher than 1 means the test reports higher throughput than NDT7.  The plot shows the consistency of the tests for both downlink and uplink directions. 

\begin{figure*}[tb!]
\begin{subfigure}[t]{.33\textwidth}
  \centering
   \captionsetup{width=.9\linewidth}
    \includegraphics[width=1\textwidth,keepaspectratio]{../figures/consistency/consistency_rel_ndt7_down.pdf}
    \caption{Downlink direction}
    \label{fig:consistency-down}
\end{subfigure}
\hfill
\begin{subfigure}[t]{.33\textwidth}
  \centering
   \captionsetup{width=.9\linewidth}
    \includegraphics[width=1\textwidth,keepaspectratio]{../figures/consistency/consistency_rel_ndt7_down_speedtier.pdf}
    \caption{Downlink direction: breakdown by speed tier}
    \label{fig:consistency-down-tier}
\end{subfigure}
\hfill
\begin{subfigure}[t]{.33\textwidth}
  \centering
   \captionsetup{width=.9\linewidth}
    \includegraphics[width=1\textwidth,keepaspectratio]{../figures/consistency/consistency_rel_ndt7_up.pdf}
    \caption{Uplink direction}
    \label{fig:consistency-up}
\end{subfigure}
\caption{Test consistency relative to NDT7}
\label{fig:consistency}
\end{figure*}

\paragraph{Results}:Figure~\ref{fig:consistency-down} shows consistency in the downlink direction.  iPerf UDP shows the highest value among the four tests.  This makes sense as UDP has no congestion control and least overhead of the tests.  Note the difference is not that significant. iPerf TCP also shows high values. This is because we filter out the slow-start.  \tarun{Check if NDT7 filters out the slow start}.  Ookla reports higher value than NDT7.  This is most likely an artifact of using multiple threads and filtering out lower percentiles of throughput from the final report.  \tarun{Check if there is consistency with in-lab measurements}

 Figure~\ref{fig:consistency-down-tier} shows the break down by speed tiers.  The difference does not change much based on the speed tier.  NDT7 can saturate high speed tier links. We also find lower consistency in  iPerf UDP for 401-800 Mbps speed tier. This suggest some weird shaping behavior for these clients. We found that the client vary in terms of their ISP. \tarun{Needs further investigation}

Figure~\ref{fig:consistency-up} shows  the consistency in the uplink direction.  Ookla,  surprisingly has a lower consistency compared to NDT7.  So does iPerf UDP.  However,  iPerf TCP has a higher throughput which could again be due to filtering the TCP slow start. 



\subsection{Effect of time of day}

\begin{figure*}[t]
	%\vspace{-10em}
    \begin{subfigure}[t]{0.33\textwidth}
    		\centering
        \includegraphics[width=\textwidth,keepaspectratio]{figures/time-of-day/ookla-down.pdf}
        \caption{Downlink - Quantization parameter}
 		\label{subfig:downlink_video_qp}
    \end{subfigure}%
    \hfill
	\begin{subfigure}[t]{0.33\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/time-of-day/ndt-down.pdf}
    \caption{Downlink - Frames per second.}
    \label{subfig:downlink_frames_per_second}
    \end{subfigure}% 
    \hfill
	\begin{subfigure}[t]{0.33\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/time-of-day/ookla-up.pdf}
    \caption{Downlink - Frame width.}
    \label{subfig:downlink_frame_width}
    \end{subfigure}
    \newline
        \begin{subfigure}[t]{0.33\textwidth}
    		\centering
        \includegraphics[width=\textwidth,keepaspectratio]{figures/time-of-day/ndt-up.pdf}
        \caption{Uplink - Quantization parameter.}
 		\label{subfig:uplink_video_qp}
    \end{subfigure}%
    \hfill
\end{figure*}

\subsection{Effect of server section}


